Dynamic System Adaptation by Constraint Orchestration

For Paradigm models, evolution is just-in-time specified coordination conducted by a special reusable component McPal. Evolution can be treated consistently and on-the-fly through Paradigm's constraint orchestration, also for originally unforeseen evolution. UML-like diagrams visually supplement such migration, as is illustrated for the case of a critical section solution evolving into a pipeline architecture.

==> df_techrep.tex <==
%% file df_malaga.tex

\newcommand{\CSM}{\textsl{CSM}}
\newcommand{\Asg}{\textsl{Asg}}
\newcommand{\Ask}{\textsl{Ask}}
\newcommand{\Check}{\textsl{Check}}
\newcommand{\Content}{\textsl{Content}}
\newcommand{\Crit}{\textsl{Crit}}
\newcommand{\Crs}{\textsl{Crs}}
\newcommand{\Crsmigr}{\textsl{Crs}_{\textit{\scriptsize migr}}}
\newcommand{\CrstoBe}{\textsl{Crs}_{\textit{\scriptsize toBe}}}
\newcommand{\Evol}{\textsl{Evol}}
\newcommand{\EvolColl}{\textsl{Evol}}
\newcommand{\EvolCoord}{\textsl{EvolCoord}}
\newcommand{\Free}{\textsl{Free}}
\newcommand{\InCS}{\textsl{InCS}}
\newcommand{\Interrupted}{\textsl{Inspec}}
\newcommand{\JITting}{\textsl{JITting}}
\newcommand{\McPal}{\textsl{McPal}}
\newcommand{\NewRuleSet}{\textsl{NewRuleSet}}
\newcommand{\MigrPhase}{\textsl{MigrPhase}}
\newcommand{\Migronetwo}{\textsl{Migr}_{1-2}}
\newcommand{\NCr}{\textsl{NCrit}}
\newcommand{\Observing}{\textsl{Observing}}
\newcommand{\OutCS}{\textsl{OutCS}}
\newcommand{\Post}{\textsl{Post}}
\newcommand{\Pre}{\textsl{Pre}}
\newcommand{\SchPhasetwo}{\textsl{Sch-Phase2}}
\newcommand{\Scheduler}{\textsl{Scheduler}}
\newcommand{\StartMigr}{\textsl{StartMigr}}
\newcommand{\StatPhase}{\textsl{StatPhase}}
\newcommand{\Unit}{\textsl{Unit}\mkern1mu}
\newcommand{\UoneWi}{\textsl{U}_1 \mbox{\texttt{:=}} \textit{W}_i}
%% \renewcommand{\UoneWi}{\textsl{U}_1 \texttt{by} \textit{W}_i}
\renewcommand{\UoneWi}{\textsl{W}_i \texttt{as} \textit{U}_1}
\newcommand{\UoneUtwoWiWj}{i: \textsl{U}_2 \texttt{by} \textsl{W}_j}
\renewcommand{\UoneUtwoWiWj}{i: \textsl{W}_j \texttt{as} \textsl{U}_2}
\newcommand{\WhoFirst}{\textsl{WhoFirst}}
\newcommand{\WiPhasetwo}{\textsl{$\textit{W}_i$-Phase2}}
\newcommand{\Worker}{\textsl{Worker}}


\newcommand{\notyet}{\textsl{notyet}}
\newcommand{\started}{\textsl{started}}
\newcommand{\triv}{\textsl{triv}}
\newcommand{\done}{\textsl{done}}



==> macros.tex <==
%% file macros.tex

% modifications of mathcode
% cf. TeX book p. 344
\mathcode`:="003A       % : ordinary symbol
\mathcode`;="203B       % ; binary symbol
\mathcode`?="003F       % ? ordinary symbol
\mathcode`|="026A       % | ordinary symbol
\mathcode`<="4268       % < abbreviates \langle
\mathcode`>="5269       % > abbreviates \rangle
                                                                                
\mathchardef\ls="213C   % less symbol (< used as \langle)
\mathchardef\gr="213E   % greater symbol (> used as \rangle)
\mathchardef\uparrow="0222      % adaptation mathmode of uparrow
\mathchardef\downarrow="0223    % adaptation mathmode of downarrow

\newcommand{\blankline}{\vspace*{\baselineskip}}
\newcommand{\halflineup}{\vspace*{-0.5\baselineskip}}

\newcommand{\ttAVAILABILITY}{\mbox{\tt AVAILABILITY}}
\newcommand{\ttCLIENT}{\mbox{\tt CLIENT}}
\newcommand{\ttCR}{\mbox{\tt CR}}
\newcommand{\ttCRhelp}{\ttCR_{\mathit{help}}}
\newcommand{\ttCRmig}{\ttCR_{\mathit{mig}}}
\newcommand{\ttCRnext}{\ttCR_{\mathit{next}}}
\newcommand{\ttCRorg}{\ttCR_{\mathit{org}}}
\newcommand{\ttMAINTENANCE}{\mbox{\tt MAINTENANCE}}
\newcommand{\ttPART}{\mbox{\tt PART}}
\newcommand{\ttSTATUS}{\mbox{\tt STATUS}}
\newcommand{\ttVAR}{\mbox{\tt var}}
\newcommand{\ttAssigned}{\mbox{\tt Assigned}}
\newcommand{\ttBroker}{\mbox{\tt Broker}}
\newcommand{\ttBusy}{\mbox{\tt Busy}}
\newcommand{\ttClient}{\mbox{\tt Client}}
\newcommand{\ttEvol}{\mbox{\tt Evol}}
\newcommand{\ttFree}{\mbox{\tt Free}}
\newcommand{\ttInCS}{\texttt{InCS}}
\newcommand{\ttMaintainer}{\mbox{\tt Maintainer}}
\newcommand{\ttMigration}{\mbox{\tt Migration}}
\newcommand{\ttMcPal}{\texttt{McPal}}
\newcommand{\ttNotAssigned}{\mbox{\tt NotAssigned}}
\newcommand{\ttNotUnderService}{\mbox{\tt WithoutService}}
\newcommand{\ttOutOfService}{\mbox{\tt OutOfService}}
\newcommand{\ttOrienting}{\mbox{\tt Orienting}}
\newcommand{\ttOutCS}{\texttt{OutCS}}
%% \newcommand{\ttPhase}{\mbox{\tt Phase}}
%% \newcommand{\ttPhaseone}{\mbox{\tt Phase}_1}
%% \newcommand{\ttPhasetwo}{\mbox{\tt Phase}_2}
\newcommand{\ttProc}{\mbox{\tt Proc}}
\newcommand{\ttProcP}{\mbox{\tt ProcP}}
\newcommand{\ttProcQ}{\mbox{\tt ProcQ}}
\newcommand{\ttReleased}{\mbox{\tt Released}}
\newcommand{\ttRunning}{\mbox{\tt Running}}
\newcommand{\ttScheduler}{\texttt{Scheduler}}
\newcommand{\ttServer}{\mbox{\tt Server}}
\newcommand{\ttSubProc}{\mbox{\tt SubProc}}
\newcommand{\ttTaken}{\mbox{\tt Taken}}
\newcommand{\ttTool}{\mbox{\tt Tool}}
\newcommand{\ttWorker}{\texttt{Worker}}
\newcommand{\ttWorkeri}{\ttWorker_i}
\newcommand{\ttWorkeriminusone}{\ttWorker_{i-1}}
\newcommand{\ttWorkeriplusone}{\ttWorker_{i+1}}
\newcommand{\ttWorkerone}{\ttWorker_1}
\newcommand{\ttUnderService}{\mbox{\tt UnderService}}
\newcommand{\ttasg}{\texttt{asg}}
\newcommand{\ttasgi}{\ttasg_i}
\newcommand{\ttasgone}{\ttasg_1}
\newcommand{\ttasgtwo}{\ttasg_2}
\newcommand{\ttasgthree}{\ttasg_3}
\newcommand{\ttasking}{\mbox{\tt asking}}
\newcommand{\ttatdesk}{\mbox{\tt at\_desk}}
\newcommand{\ttcheck}{\mbox{\tt check}}
\newcommand{\ttchecki}{\ttcheck_i}
\newcommand{\ttcheckiplusone}{\ttcheck_{i+1}}
\newcommand{\ttcheckone}{\ttcheck_1}
\newcommand{\ttcheckthree}{\ttcheck_3}
\newcommand{\ttchecktwo}{\ttcheck_2}
\newcommand{\ttbusy}{\mbox{\tt busy}}
\newcommand{\ttclient}{\mbox{\tt client}}
\newcommand{\ttcontinuemigration}{\texttt{contMigr}}
\newcommand{\ttcritical}{\texttt{crit}}
\newcommand{\ttdone}{\texttt{done}}
\newcommand{\ttendmigration}{\texttt{endMigr}}
\newcommand{\ttentering}{\texttt{entering}}
\newcommand{\ttexpr}{\texttt{expr}}
\newcommand{\ttfree}{\mbox{\tt free}}
\newcommand{\ttfollowup}{\texttt{post}}
\newcommand{\ttidle}{\mbox{\tt idle}}
\newcommand{\ttleft}{\texttt{left}}
\newcommand{\ttmediate}{\mbox{\tt mediate}}
\newcommand{\ttmaintenance}{\mbox{\tt maint}}
\newcommand{\ttneedclear}{\mbox{\tt need\_clear}}
\newcommand{\ttnoneeds}{\mbox{\tt no\_needs}}
\newcommand{\ttnoncritical}{\texttt{nonCrit}}
\newcommand{\ttnomaintenance}{\mbox{\tt no\_maint}}
\newcommand{\ttobs}{\texttt{obs}}
\newcommand{\ttpreparation}{\texttt{pre}}
\newcommand{\ttstartmigration}{\texttt{startMigr}}
\newcommand{\ttstatea}{\mbox{\tt state\_a}}
\newcommand{\ttstateb}{\mbox{\tt state\_b}}
\newcommand{\tttoBeReleased}{\mbox{\tt toBeReleased}}
\newcommand{\tttoBeTaken}{\mbox{\tt toBeTaken}}
\newcommand{\ttoccupied}{\mbox{\tt occupied}}
\newcommand{\ttready}{\mbox{\tt ready}}
\newcommand{\ttsatisfied}{\mbox{\tt satisfied}}
\newcommand{\ttserve}{\mbox{\tt serve}}
\newcommand{\ttserverClear}{\mbox{\tt serverClear}}
\newcommand{\ttstalled}{\mbox{\tt stalled}}
\newcommand{\ttstarted}{\texttt{started}}
\newcommand{\ttstatus}{\mbox{\tt status}}
\newcommand{\tttriv}{\mbox{\tt triv}}
\newcommand{\ttunderservice}{\mbox{\tt service}}

\newcommand{\AL}{\mbox{\tt AC}}
\newcommand{\ST}{\mbox{\tt ST}}
\newcommand{\LB}{\mbox{\tt LB}}
\newcommand{\TS}{\mbox{\tt TS}}
\newcommand{\lb}{\mbox{\tt lb}}
\newcommand{\al}{\mbox{\tt ac}}
\newcommand{\st}{\mbox{\tt st}}
\renewcommand{\ts}{\mbox{\tt ts}}
\newcommand{\alprime}{\al'}
\newcommand{\stprime}{\st'}
\newcommand{\tsprime}{\ts'}
\newcommand{\lbprime}{\lb'}

\newcommand{\arrow}[2]{\,{{\stackrel{#2}{\rightarrow}}_{#1}}\,}
\newcommand{\notarrow}[2]{\,{{\stackrel{#2}{\nrightarrow}}_{#1}}\,}
\newcommand{\aarrow}{\arrow{}{a}}
\newcommand{\aiarrow}{\arrow{}{a_i}}
\newcommand{\thetaonearrow}{\arrow{}{\theta_1}}
\newcommand{\thetanarrow}{\arrow{}{\theta_n}}
\newcommand{\thetanotarrow}{\notarrow{}{\theta}}

\newcommand{\To}{\Longrightarrow}
\newcommand{\assign}{\mathrel{\, \texttt{:=} \,}}
\newcommand{\crmarker}{\mathrel{\ast}}
\newcommand{\lc}{\lbrace\:}
\newcommand{\myast}{\; \crmarker \;}
\newcommand{\nilarrow}{\to}
\newcommand{\notto}{\not\to}
\newcommand{\rc}{\:\rbrace}
\newcommand{\setH}{\lbrace H \rbrace}
\newcommand{\setHij}{\lbrace H + (i,j) \rbrace}

\newcommand{\addressarrow}{\arrow{}{address(i)}}
\newcommand{\askingarrow}{\arrow{}{asking}}
\newcommand{\leavearrow}{\arrow{}{leave(i)}}
\newcommand{\questioncleararrow}{\arrow{}{serverClear}}
\newcommand{\enterarrow}{\arrow{}{enter}}
\newcommand{\explainarrow}{\arrow{}{explain}}

%% old df_malaga.tex incorported from df_coord06.tex

\newcommand{\AC}{\mbox{\tt AC}}
%%\newcommand{\AT}{\mbox{\tt AT}}
\newcommand{\ATi}{\AT_i}
\newcommand{\ATn}{\AT_n}
\newcommand{\ATone}{\AT_1}
\newcommand{\CT}{\mbox{\tt CT}}
\newcommand{\GAC}{\mbox{\tt GAC}}
\newcommand{\GAL}{\mbox{\tt GAL}}
\newcommand{\GST}{\mbox{\tt GST}}
\newcommand{\GTS}{\mbox{\tt GTS}}
%%\newcommand{\LB}{\mbox{\tt LB}}
\newcommand{\LBi}{\LB_i}
\newcommand{\PT}{\mbox{\tt PT}}
\newcommand{\PTi}{\PT_i}
%%\newcommand{\ST}{\mbox{\tt ST}}
\newcommand{\STi}{\ST_i}
\newcommand{\TR}{\mbox{\tt TR}}
\newcommand{\TRi}{\TR_i}
%%\newcommand{\TS}{\mbox{\tt TS}}
\newcommand{\TSi}{\TS_i}
\newcommand{\ac}{\mbox{\tt ac}}
\newcommand{\acprime}{\ac'}
\newcommand{\aci}{\ac_i}
%%\newcommand{\at}{\mbox{\tt at}}
%%\newcommand{\ati}{\at_i}
%%\newcommand{\lb}{\mbox{\tt lb}}
\newcommand{\lbi}{\lb_i}
%%\newcommand{\lbprime}{\lb'}
\newcommand{\man}{\mbox{\tt man}}
\newcommand{\ok}{\mbox{\tt ok}}
\newcommand{\pr}{\mbox{\tt pr}}
\renewcommand{\sp}{\tt sp}
\newcommand{\spprime}{\sp'}
%%newcommand{\st}{\mbox{\tt st}}
%%\newcommand{\stprime}{\st'}
\newcommand{\stc}{\st_c}
\newcommand{\stci}{\st_c^i}
\newcommand{\stcnod}{\st_c^0}
\newcommand{\stcone}{\st_c^1}
\newcommand{\sti}{\st_i}
\newcommand{\stp}{\st_p}
\newcommand{\sys}{\mbox{\tt sys}}
\newcommand{\tr}{\mbox{\tt tr}}
\newcommand{\trap}{\mbox{\tt trap}}
\newcommand{\trc}{\tr_c}
\newcommand{\trcnod}{\tr_c^0}
\newcommand{\trcone}{\tr_c^1}
\newcommand{\trci}{\tr_c^i}
\newcommand{\tri}{\tr_i}
%%\newcommand{\ts}{\mbox{\tt ts}}
%%\newcommand{\tsprime}{\ts'}
\newcommand{\tsc}{\ts_c}
\newcommand{\tsci}{\ts_c^i}
\newcommand{\tscnod}{\ts_c^0}
\newcommand{\tscone}{\ts_c^1}
\newcommand{\tsi}{\ts_i}
\newcommand{\tsp}{\ts_p}

\newcommand{\slAny}{\mbox{\sl Any}}
\newcommand{\slB}{\mbox{\sl B}}
\newcommand{\slC}{\mbox{\sl C}}
\newcommand{\slCPUQ}{\mbox{\sl CPUQ}}
\newcommand{\slIn}{\mbox{\sl In}}
\newcommand{\slCheckOK}{\mbox{\sl CheckOK}}
\newcommand{\slCheckKO}{\mbox{\sl CheckKO}}
\newcommand{\slDone}{\mbox{\sl Done}}
\newcommand{\slFull}{\mbox{\sl Full}}
\newcommand{\slFree}{\mbox{\sl Free}}
\newcommand{\slGetPaint}{\mbox{\sl GetPaint}}
\newcommand{\slOut}{\mbox{\sl Out}}
\newcommand{\slP}{\mbox{\sl P}}
\newcommand{\slPone}{\slP_1}
\newcommand{\slPtwo}{\slP_2}
\newcommand{\slPaintB}{\mbox{\sl PaintB}}
\newcommand{\slPaintR}{\mbox{\sl PaintR}}
\newcommand{\slPU}{\mbox{\sl PU}}
\newcommand{\slQ}{\mbox{\sl Q}}
\newcommand{\slR}{\mbox{\sl R}}
\newcommand{\slRequest}{\mbox{\sl Request}}
\newcommand{\slS}{\mbox{\sl S}}
\newcommand{\slSone}{\slS_1}
\newcommand{\slStwo}{\slS_2}
\newcommand{\slSthree}{\slS_3}
\newcommand{\slSpot}{\mbox{\sl S}}
\newcommand{\slSpotone}{\slSpot_1}
\newcommand{\slSpottwo}{\slSpot_2}
\newcommand{\slSpotthree}{\slSpot_3}
\newcommand{\slcheck}{\mbox{\sl check}}
\newcommand{\sldo}{\mbox{\sl do}}
\newcommand{\sldone}{\mbox{\sl done}}
\newcommand{\slidle}{\mbox{\sl idle}}
\newcommand{\slin}{\mbox{\sl in}}
\newcommand{\slpainted}{\mbox{\sl painted}}
\newcommand{\slprep}{\mbox{\sl prep}}
\newcommand{\slpu}{\mbox{\sl pu}}
\newcommand{\slpufive}{\slpu_5}
\newcommand{\slpufour}{\slpu_4}
\newcommand{\slpui}{\slpu_i}
\newcommand{\slpuj}{\slpu_j}
\newcommand{\slpunod}{\slpu_0}
\newcommand{\slpuone}{\slpu_1}
\newcommand{\slputhree}{\slpu_3}
\newcommand{\slputwo}{\slpu_2}
\newcommand{\slreqB}{\mbox{\sl reqB}}
\newcommand{\slreqR}{\mbox{\sl reqR}}
\newcommand{\slstart}{\mbox{\sl start}}
\newcommand{\sltriv}{\mbox{\sl triv}}

\newcommand{\AllSafe}{\mbox{\sl AllSafe}}
\newcommand{\Buffertwo}{\mbox{\sl Buffer}_2}
\newcommand{\Cons}{\mbox{\sl Cons}}
\newcommand{\ConsCaptwo}{\mbox{\sl ConsCap}_2}
\newcommand{\FromOneToTwo}{\mbox{\sl From1to2}}
\newcommand{\CCrit}{\mbox{\sl CCrit}}
\newcommand{\CSafe}{\mbox{\sl CSafe}}
\newcommand{\PCrit}{\mbox{\sl PCrit}}
\newcommand{\PSafe}{\mbox{\sl PSafe}}
%% \newcommand{\Phaseone}{\mbox{\sl Phase}_1}
%% \newcommand{\Phasetwo}{\mbox{\sl Phase}_2}
%% \newcommand{\Phasethree}{\mbox{\sl Phase}_3}
\newcommand{\Presentone}{\mbox{\sl Present}_1}
\newcommand{\Prod}{\mbox{\sl Prod}}
\newcommand{\ProdCaptwo}{\mbox{\sl ProdCap}_2}
\newcommand{\Spot}{\mbox{\sl Spot}}
%% \newcommand{\Subpr}{\mbox{\sl Subpr}}
\newcommand{\TentCons}{\mbox{\sl TentCons}}
\newcommand{\TentProd}{\mbox{\sl TentProd}}
\newcommand{\ToCrit}{\mbox{\sl ToCrit}}
\newcommand{\ToSafe}{\mbox{\sl ToSafe}}
\newcommand{\UnitB}{\mbox{\sl Unit~B}}
\newcommand{\UnitR}{\mbox{\sl Unit~R}}
\newcommand{\Usedone}{\mbox{\sl Used}_1}
\newcommand{\Usedthree}{\mbox{\sl Used}_3}
\newcommand{\cons}{\mbox{\sl cons}}
\newcommand{\cs}{\mbox{\sl cons}}
\newcommand{\myempty}{\mbox{\sl empty}}
\newcommand{\myfill}{\mbox{\sl fill}}
\newcommand{\gotone}{\mbox{\sl gotone}}
\newcommand{\gotonei}{\gotone_i}
\newcommand{\gt}{\mbox{\sl empty}}
\newcommand{\myskip}{\mbox{\sl skip}}
\newcommand{\none}{\mbox{\sl none}}
\newcommand{\nonei}{\none_i}
\newcommand{\noneiplusone}{\none_{i+1}}
%%\newcommand{\ok}{\mbox{\sl ok}}
\newcommand{\one}{\mbox{\sl one}}
\newcommand{\oneCCrit}{1\CCrit}
\newcommand{\oneConePCrit}{1\mbox{\sl C}\&1\PCrit}
\newcommand{\onePCrit}{1\PCrit}
\newcommand{\onei}{\one_i}
\newcommand{\pd}{\mbox{\sl prod}}
\newcommand{\producer}{\mbox{\sl prod}}
\newcommand{\pt}{\mbox{\sl pt}}
%% \newcommand{\subpr}{\mbox{\sl subpr}}

\newcommand{\ssFromOneToTwo}{\mbox{\scriptsize\sl FromOneToTwo}}
\newcommand{\sscheck}{\mbox{\scriptsize\sl check}}
\newcommand{\sscs}{\mbox{\scriptsize\sl cons}}
\newcommand{\ssconsume}{\mbox{\scriptsize\sl consume}}
%%\newcommand{\ssdone}{\mbox{\scriptsize\sl done}}
\newcommand{\ssdoi}{\mbox{\scriptsize\sl do} \mkern 1mu (i)}
\newcommand{\ssdotwo}{\mbox{\scriptsize\sl do} \mkern 1mu (2)}
\newcommand{\ssempty}{\mbox{\scriptsize\sl empty}}
\newcommand{\ssgt}{\mbox{\scriptsize\sl empty}}
\newcommand{\ssok}{\mbox{\scriptsize\sl ok}}
\newcommand{\ssidle}{\mbox{\scriptsize\sl idle}}
\newcommand{\sspainted}{\mbox{\scriptsize\sl painted}}
\newcommand{\sspd}{\mbox{\scriptsize\sl prod}}
\newcommand{\ssprep}{\mbox{\scriptsize\sl prep}}
\newcommand{\sspt}{\mbox{\scriptsize\sl fill}}
\newcommand{\ssreqB}{\mbox{\scriptsize\sl reqB}}
\newcommand{\ssreqR}{\mbox{\scriptsize\sl reqR}}
\newcommand{\ssskip}{\mbox{\scriptsize\sl skip}}
\newcommand{\ssstart}{\mbox{\scriptsize\sl start}}
%%\newcommand{\ssstarted}{\mbox{\scriptsize\sl started}}
\newcommand{\sstriv}{\mbox{\scriptsize\sl triv}}
\newcommand{\sstrivial}{\mbox{\scriptsize\sl triv}}
\newcommand{\sstv}{\mbox{\scriptsize\sl triv}}
%%\newcommand{\trap}{\mbox{\sl trap}}
\newcommand{\striv}{\mbox{\sl triv}}
\newcommand{\trivi}{\striv_i}
\newcommand{\trivj}{\striv_j}
\newcommand{\tv}{\mbox{\sl triv}}
\newcommand{\twoCCrit}{2\CCrit}
\newcommand{\twoPCrit}{2\PCrit}

\newcommand{\calE}{\mbox{$\cal E$}}
\newcommand{\calEone}{\calE_1}
\newcommand{\calEi}{\calE_i}
\newcommand{\calEn}{\calE_n}
\newcommand{\calM}{\mbox{$\cal M$}}
\newcommand{\calP}{\mbox{$\cal P$}}

\newcommand{\Cinodinfty}{\brace C_i \rbrace_{i=0}^\infty}
\newcommand{\Dij}{D_{i,j}}
\newcommand{\If}{\mathrel{\Leftarrow}}
\newcommand{\Sij}{S_{i,j}}
\newcommand{\Sijprime}{S'_{i,j}}
\newcommand{\Sinodinfty}{(S_i)_{i=0}^\infty}
\newcommand{\Skj}{S_{k,j}}
\newcommand{\sioneton}{(s_i)_{i=1}^n}
\newcommand{\siprimeoneton}{(s'_i)_{i=1}^n}
\newcommand{\tij}{t_{i,j}}

\newcommand{\implies}{\mathrel{\Rightarrow}}
\newcommand{\la}{\langle\,}
\newcommand{\lbb}{\mathopen{[\![}}
%%\newcommand{\lc}{\lbrace\:}
\newcommand{\lconetomrc}{\lc 1, \ldots, m \rc}
\newcommand{\lconetonrc}{\lc 1, \ldots, n \rc}
\newcommand{\pijSjthetaj}{\pi_{j}(S_j,\theta_j)}
\newcommand{\piijSijthetaij}{\pi_{i,j}(S_{i,j},\theta_{i,j})}
\newcommand{\piijSijprimethetaijprime}{\pi_{i,j}(S'_{i,j},\theta'_{i,j})}
\newcommand{\piij}{\pi_{i,j}}
\newcommand{\pionejjinJone}{( \pi_{1,j} )_{j \in J_1}}
\newcommand{\piijjinJi}{( \pi_{i,j} )_{j \in J_i}}
\newcommand{\pinjjinJn}{( \pi_{n,j} )_{j \in J_n}}
\newcommand{\placeholder}[1]{[#1]}
\newcommand{\powerset}{\calP}
\newcommand{\ra}{\,\rangle}
%%\newcommand{\rc}{\:\rbrace}
\newcommand{\rbb}{\mathclose{]\!]}}
\newcommand{\semicolon}{\mathclose{;\ }}
\newcommand{\singleton}[1]{\lbrace #1 \rbrace}
\newcommand{\state}[1]{\lbb#1\rbb}
\newcommand{\thetaij}{\theta_{i,j}}


\newcommand{\Piij}{\Pi_{i,j}}
\newcommand{\Piizero}{\Pi_{i,0}}
\newcommand{\Sigmaij}{\Sigma_{i,j}}


%%\newcommand{\arrow}[2]{\,{{\stackrel{#2}{\rightarrow}}_{#1}}\,}
\newcommand{\longarrow}[2]{\,{{\stackrel{#2}{\joinrel\rightarrow}}_{#1}}\,}
\newcommand{\FromOneToTwoarrow}{\arrow{}{\ssFromOneToTwo}}
%%\newcommand{\aarrow}{\arrow{}{a}}
%%\newcommand{\aiarrow}{\arrow{}{a_i}}
%%\newcommand{\nilarrow}{\arrow{}{}}
\newcommand{\nilarrowast}{\to^\ast}
\newcommand{\checkarrow}{\arrow{}{\sscheck}}
\newcommand{\csarrow}{\arrow{}{\sscs}}
\newcommand{\consumearrow}{\longarrow{}{\ssconsume}}
\newcommand{\doiarrow}{\arrow{}{\ssdoi}}
%%\newcommand{\donearrow}{\arrow{}{\ssdone}}
\newcommand{\dotwoarrow}{\arrow{}{\ssdotwo}}
\newcommand{\emptyarrow}{\longarrow{}{\ssempty}}
\newcommand{\gtarrow}{\arrow{}{\ssgt}}
\newcommand{\idlearrow}{\arrow{}{\ssidle}}
\newcommand{\okonearrow}{\arrow{}{\ssok_1}}
\newcommand{\oktwoarrow}{\arrow{}{\ssok_2}}
\newcommand{\paintedarrow}{\arrow{}{\sspainted}}
\newcommand{\pdarrow}{\arrow{}{\sspd}}
\newcommand{\preparrow}{\arrow{}{\ssprep}}
\newcommand{\ptarrow}{\arrow{}{\sspt}}
\newcommand{\reqBarrow}{\arrow{}{\ssreqB}}
\newcommand{\reqRarrow}{\arrow{}{\ssreqR}}
\newcommand{\startarrow}{\arrow{}{\ssstart}}
\newcommand{\startednotarrow}{\notarrow{}{\ssstarted}}
\newcommand{\tarrow}{\arrow{}{t}}

\newcommand{\thetaarrow}{\arrow{}{\theta}}
\newcommand{\thetaeparrow}{\arrow{}{\theta_{e,p}}}
\newcommand{\thetafqarrow}{\arrow{}{\theta_{f,q}}}
\newcommand{\thetaep}{\theta_{e,p}}
\newcommand{\thetafq}{\theta_{f,q}}

\newcommand{\thetaijarrow}{\arrow{}{\thetaij}}
\newcommand{\trivarrow}{\arrow{}{\sstriv}}
\newcommand{\thetahatijarrow}{\arrow{}{\hat{\theta}_{i,j}}}
\newcommand{\tiarrow}{\arrow{}{t_i}}
\newcommand{\tnarrow}{\arrow{}{t_n}}
\newcommand{\tonearrow}{\arrow{}{t_1}}
\newcommand{\trivialarrow}{\longarrow{}{\sstrivial}}
%%\newcommand{\trivarrow}{\arrow{}{\sstrivial}}
\newcommand{\tthreearrow}{\arrow{}{t_3}}
\newcommand{\ttwoarrow}{\arrow{}{t_2}}
\newcommand{\tvonearrow}{\arrow{}{\sstv_1}}
\newcommand{\tvtwoarrow}{\arrow{}{\sstv_2}}

\newcommand{\negarrow}[2]{\,{{\stackrel{#2}{\nrightarrow}}_{#1}}\,}
\newcommand{\reqBnegarrow}{\negarrow{}{\ssreqB}}
\newcommand{\reqRnegarrow}{\negarrow{}{\ssreqR}}
\newcommand{\startednegarrow}{\negarrow{}{\ssstarted}}
\newcommand{\thetanegarrow}{\negarrow{}{\theta}}



\newcommand{\gtdownarrow}{\phantom{\, \ssgt} \downarrow \, \ssgt}
\newcommand{\csdownarrow}{\phantom{\, \sscs} \downarrow \, \sscs}


%% new commands for afterfsen

\newcommand{\ssaccept}{\mbox{\scriptsize\sl accept}}
%%\newcommand{\ssall}{\mbox{\scriptsize\sl all}}
\newcommand{\ssallow}{\mbox{\scriptsize\sl allow}}
\newcommand{\ssannounce}{\mbox{\scriptsize\sl announce}}
\newcommand{\ssask}{\mbox{\scriptsize\sl ask}}
\newcommand{\ssbegin}{\mbox{\scriptsize\sl begin}}
%%\newcommand{\sscheck}{\mbox{\scriptsize\sl check}}
\newcommand{\sscontinue}{\mbox{\scriptsize\sl continue}}
%%\newcommand{\ssctn}{\mbox{\scriptsize\sl ctn}}
\newcommand{\ssdeliver}{\mbox{\scriptsize\sl deliver}}
\newcommand{\ssdisallow}{\mbox{\scriptsize\sl disallow}}
%%\newcommand{\ssdne}{\mbox{\scriptsize\sl dne}}
\newcommand{\ssdone}{\mbox{\scriptsize\sl done}}
\newcommand{\ssenjoying}{\mbox{\scriptsize\sl enjoying}}
\newcommand{\ssfinish}{\mbox{\scriptsize\sl finish}}
\newcommand{\ssfixatearch}{\mbox{\scriptsize\sl fixateArch}}
\newcommand{\ssfreezepipeline}{\mbox{\scriptsize\sl freezePipeline}}
\newcommand{\ssgiveout}{\mbox{\scriptsize\sl giveOut}}
\newcommand{\ssgrant}{\mbox{\scriptsize\sl grant}}
\newcommand{\ssgreet}{\mbox{\scriptsize\sl greet}}
\newcommand{\ssimprove}{\mbox{\scriptsize\sl improve}}
\newcommand{\ssinterruptable}{\mbox{\scriptsize\sl interruptable}}
\newcommand{\sskickoff}{\mbox{\scriptsize\sl kickOff}}
\newcommand{\ssknowchange}{\mbox{\scriptsize\sl knowChange}}
\newcommand{\sslaydown}{\mbox{\scriptsize\sl layDown}}
\newcommand{\ssleeve}{\mbox{\scriptsize\sl leave}}
\newcommand{\ssmigrate}{\mbox{\scriptsize\sl migrate}}
\newcommand{\ssmigrdone}{\mbox{\scriptsize\sl migrDone}}
\newcommand{\ssnevermore}{\mbox{\scriptsize\sl neverMore}}
\newcommand{\ssnotyet}{\mbox{\scriptsize\sl notYet}}
%%\newcommand{\ssnyt}{\mbox{\scriptsize\sl nYt}}
\newcommand{\ssoccupy}{\mbox{\scriptsize\sl occupy}}
\newcommand{\ssoffer}{\mbox{\scriptsize\sl offer}}
\newcommand{\ssoncemore}{\mbox{\scriptsize\sl onceMore}}
\newcommand{\ssonitsway}{\mbox{\scriptsize\sl onItsWay}}
\newcommand{\sspass}{\mbox{\scriptsize\sl pass}}
\newcommand{\sspause}{\mbox{\scriptsize\sl pause}}
\newcommand{\sspermit}{\mbox{\scriptsize\sl permit}}
\newcommand{\ssphaseauto}{\mbox{\scriptsize\sl phaseAuto}}
\newcommand{\ssphaseout}{\mbox{\scriptsize\sl phaseOut}}
\newcommand{\sspickup}{\mbox{\scriptsize\sl pickUp}}
\newcommand{\ssproceed}{\mbox{\scriptsize\sl proceed}}
\newcommand{\ssproduce}{\mbox{\scriptsize\sl produce}}
\newcommand{\sspseudoenjoying}{\mbox{\scriptsize\sl pseudoEnjoying}}
\newcommand{\sspseudointerruptable}{\mbox{\scriptsize\sl pseudoInterruptable}}
\newcommand{\sspseudotrivasunit}{\mbox{\scriptsize\sl pseudoTrivAsUnit}}
\newcommand{\ssready}{\mbox{\scriptsize\sl ready}}
\newcommand{\ssreadydefault}{\mbox{\scriptsize\sl readyDefault}}
\newcommand{\ssreadynondefault}{\mbox{\scriptsize\sl readyNonDefault}}
\newcommand{\ssreadyforfour}{\mbox{\scriptsize\sl readyFor4}}
%%\newcommand{\ssreq}{\mbox{\scriptsize\sl req}}
\newcommand{\ssrefuse}{\mbox{\scriptsize\sl refuse}}
\newcommand{\ssrequest}{\mbox{\scriptsize\sl request}}
\newcommand{\ssrestarted}{\mbox{\scriptsize\sl restarted}}
%%\newcommand{\ssrqw}{\mbox{\scriptsize\sl rqW}}
\newcommand{\ssseeworker}{\mbox{\scriptsize\sl seeWorker}}
\newcommand{\ssseeworkeri}
  {\mbox{\scriptsize\sl seeWorker}_{\mbox{\tiny\sl \,i}}}
\newcommand{\ssseeworkerj}
  {\mbox{\scriptsize\sl seeWorker}_{\mbox{\tiny\sl \,j}}}
\newcommand{\ssstarted}{\mbox{\scriptsize\sl started}}
\newcommand{\ssstartothers}{\mbox{\scriptsize\sl startOthers}}
\newcommand{\sstake}{\mbox{\scriptsize\sl take}}
\newcommand{\ssthank}{\mbox{\scriptsize\sl thank}}
\newcommand{\sstowardsdefault}{\mbox{\scriptsize\sl towardsDefault}}
%%\newcommand{\sstrv}{\mbox{\scriptsize\sl trv}}
\newcommand{\sswantchange}{\mbox{\scriptsize\sl wantChange}}
\newcommand{\sswelcoming}{\mbox{\scriptsize\sl welcoming}}

\newcommand{\acceptarrow}{\arrow{}{\ssaccept}}
%%\newcommand{\allarrow}{\arrow{}{\ssall}}
\newcommand{\allowarrow}{\arrow{}{\ssallow}}
\newcommand{\allowiarrow}{\arrow{}{\ssallow_i}}
\newcommand{\announcearrow}{\arrow{}{\ssannounce}}
\newcommand{\askkarrow}{\arrow{}{\ssask_k}}
\newcommand{\beginarrow}{\arrow{}{\ssbegin}}
\newcommand{\checkiarrow}{\arrow{}{\sscheck_i}}
\newcommand{\continuearrow}{\arrow{}{\sscontinue}}
%%\newcommand{\ctnarrow}{\arrow{}{\ssctn}}
\newcommand{\deliverarrow}{\arrow{}{\ssdeliver}}
\newcommand{\disallowarrow}{\arrow{}{\ssdisallow}}
%%\newcommand{\dnearrow}{\arrow{}{\ssdne}}
\newcommand{\donearrow}{\arrow{}{\ssdone}}
\newcommand{\enjoyingarrow}{\arrow{}{\ssenjoying}}
\newcommand{\finisharrow}{\arrow{}{\ssfinish}}
\newcommand{\fixatearcharrow}{\arrow{}{\ssfixatearch}}
\newcommand{\freezepipelinearrow}{\arrow{}{\ssfreezepipeline}}
\newcommand{\giveoutarrow}{\arrow{}{\ssgiveout}}
\newcommand{\greetarrow}{\arrow{}{\ssgreet}}
\newcommand{\grantarrow}{\arrow{}{\ssgrant}}
\newcommand{\improvearrow}{\arrow{}{\ssimprove}}
\newcommand{\interruptablearrow}{\arrow{}{\ssinterruptable}}
\newcommand{\kickoffarrow}{\arrow{}{\sskickoff}}
\newcommand{\knowchangearrow}{\arrow{}{\ssknowchange}}
\newcommand{\laydownarrow}{\arrow{}{\sslaydown}}
\newcommand{\leevearrow}{\arrow{}{\ssleeve}}
\newcommand{\migratearrow}{\arrow{}{\ssmigrate}}
\newcommand{\migrdonearrow}{\arrow{}{\ssmigrdone}}
\newcommand{\nevermorearrow}{\arrow{}{\ssnevermore}}
\newcommand{\notyetarrow}{\arrow{}{\ssnotyet}}
%%\newcommand{\nytarrow}{\arrow{}{\ssnyt}}
\newcommand{\occupyarrow}{\arrow{}{\ssoccupy}}
\newcommand{\offerarrow}{\arrow{}{\ssoffer}}
\newcommand{\oncemorearrow}{\arrow{}{\ssoncemore}}
\newcommand{\onitswayarrow}{\arrow{}{\ssonitsway}}
\newcommand{\passarrow}{\arrow{}{\sspass}}
\newcommand{\permitarrow}{\arrow{}{\sspermit}}
\newcommand{\phaseautoarrow}{\arrow{}{\ssphaseauto}}
\newcommand{\phaseoutarrow}{\arrow{}{\ssphaseout}}
\newcommand{\pickuparrow}{\arrow{}{\sspickup}}
\newcommand{\proceedarrow}{\arrow{}{\ssproceed}}
\newcommand{\producearrow}{\arrow{}{\ssproduce}}
\newcommand{\pseudoenjoyingarrow}{\arrow{}{\sspseudoenjoying}}
\newcommand{\pseudointerruptablearrow}{\arrow{}{\sspseudointerruptable}}
\newcommand{\pseudotrivasunittwoarrow}{\arrow{}{\sspseudotrivasunit_2}}
\newcommand{\readyarrow}{\arrow{}{\ssready}}
\newcommand{\readydefaultarrow}{\arrow{}{\ssreadydefault}}
\newcommand{\readynondefaultarrow}{\arrow{}{\ssreadynondefault}}
\newcommand{\readyforfourarrow}{\arrow{}{\ssreadyforfour}}
%%\newcommand{\reqarrow}{\arrow{}{\ssreq}}
\newcommand{\refusearrow}{\arrow{}{\ssrefuse}}
\newcommand{\requestarrow}{\arrow{}{\ssrequest}}
\newcommand{\restartedarrow}{\arrow{}{\ssrestarted}}
%%\newcommand{\rqwkarrow}{\arrow{}{\ssrqw_k}}
\newcommand{\seeworkeriarrow}{\arrow{}{\ssseeworkeri}}
\newcommand{\seeworkerjarrow}{\arrow{}{\ssseeworkerj}}
\newcommand{\startedarrow}{\arrow{}{\ssstarted}}
\newcommand{\takearrow}{\arrow{}{\sstake}}
\newcommand{\thankarrow}{\arrow{}{\ssthank}}
\newcommand{\towardsdefaultarrow}{\arrow{}{\sstowardsdefault}}
%%\newcommand{\trvarrow}{\arrow{}{\sstrv}}
\newcommand{\wantchangearrow}{\arrow{}{\sswantchange}}
\newcommand{\welcomingarrow}{\arrow{}{\sswelcoming}}



\newcommand{\Client}{\textsf{Client}}
\newcommand{\CS}{\textsf{CS}}
\newcommand{\CSND}{\textsf{CSNDet}}
\newcommand{\CSRR}{\textsf{CSRoRo}}
\newcommand{\NDetServer}{\textsf{NDetServer}}
\newcommand{\RoRoServer}{\textsf{RoRoServer}}
\newcommand{\Server}{\textsf{Server}}
\newcommand{\Shop}{\textsf{Shop}}
\newcommand{\ShopND}{\textsf{Shop-NonDeterministic}}
\newcommand{\ShopRR}{\textsf{Shop-RoundRobin}}

\newcommand{\AtDoor}{\textsf{AtDoor}}
\newcommand{\Busy}{\textsf{Busy}}
\newcommand{\Checking}{\textsf{Checking}}
\newcommand{\Helping}{\textsf{Helping}}
\newcommand{\Idle}{\textsf{Idle}}
\newcommand{\In}{\textsf{In}}
\newcommand{\Interrupt}{\textsf{Interrupt}}
\newcommand{\NDChecking}{\textsf{NDChecking}}
\newcommand{\NDHelping}{\textsf{NDHelping}}
\newcommand{\Out}{\textsf{Out}}
\newcommand{\RRChecking}{\textsf{RRChecking}}
\newcommand{\RRHelping}{\textsf{RRHelping}}
\newcommand{\Waiting}{\textsf{Waiting}}
\newcommand{\With}{\textsf{With}}
\newcommand{\Without}{\textsf{Without}}


%\newcommand{\address}{\textsf{address}}
\newcommand{\allow}{\textsf{allow}}
\newcommand{\checki}{\textsf{check}}
\newcommand{\continue}{\textsf{continue}}
\newcommand{\disallow}{\textsf{disallow}}
\newcommand{\enter}{\textsf{enter}}
\newcommand{\explain}{\textsf{explain}}
\newcommand{\grant}{\textsf{grant}}
\newcommand{\leave}{\textsf{leave}}
\newcommand{\pass}{\textsf{pass}}
\newcommand{\permit}{\textsf{permit}}
\newcommand{\proceed}{\textsf{proceed}}
\newcommand{\refuse}{\textsf{refuse}}
\newcommand{\request}{\textsf{request}}
\newcommand{\thank}{\textsf{thank}}

\newcommand{\CSMColl}{\textsl{CSMColl}}

\newcommand{\ProdCons}{\textsl{ProdCons}}
\newcommand{\Conf}{\textsl{Conf}}
\newcommand{\WorkerToBeUnit}{\textsl{WorkerToBeUnit}}
\newcommand{\onItsWay}{\textsl{onItsWay}}
\newcommand{\TowardsUnit}{\textsl{TowardsUnit}\mkern1mu}
\newcommand{\Phase}{\textsl{OrigAsWorker}}
\newcommand{\OrigAsSched}{\textsl{OrigAsSched}}
\newcommand{\PhasetwoAsUnit}{\textsl{ToBeAsUnit}}
\newcommand{\PhasetwoAsUnitone}{\textsl{ToBeAsUnit}_1}
\newcommand{\PhasetwoAsUnittwo}{\textsl{ToBeAsUnit}_2}
\newcommand{\PhasetwoAsUnitthree}{\textsl{ToBeAsUnit}_3}
\newcommand{\PhasetwoAsUnitfour}{\textsl{ToBeAsUnit}_4}
\newcommand{\migrDone}{\textsl{migrDone}}
\newcommand{\ready}{\textsl{ready}}
\newcommand{\W}{\textsl{W}}
\newcommand{\Cfr}{\textsl{Cfr}}
\newcommand{\consrule}{\textsl{cr}}
\newcommand{\expr}{\textsl{expr}}





%% additions Malaga %%



==> sec4.tex <==
%% file sec4.tex

\section{Conclusion}

To cater for future, unforeseen on-the-fly migration, $\McPal$ can be
incorporated into any Paradigm model. 
% $\McPal$ provides a pattern for dynamic evolution management in a
% distributed constellation of the architecture.
$\McPal$ comprises the coordination needed for
conducting the migration collaboration of all components towards a new
way of working.  Modeled just-in-time, migration coordination is such
that no form of temporary quiescence is needed to occur for whatever
component during its migration. Any such component remains in
execution, be it in a smoothly changing manner, gradually adapting to
new circumstances arising along the migration trajectory. $\McPal$'s
coordination, as specified in Paradigm, maintains consistency of the
model both during and after migration, thereby dealing with the
various dynamic consistency problem types. It is noted, UML
visualizations substantially supplement the understanding of the
evolution.  In this manner, McPal is capable to coordinate its own
migration trajectory dynamically consistent with the other components.

$\McPal$ as introduced here, generalizes the McPal
from~\cite{coord06}, as now it allows all kinds of complex behaviour
in the JIT modeled phase $\MigrPhase$, as long as it remains a correct
Paradigm coordination. The McPal component proposed in~\cite{coord06}
was restricted to a fixed migration coordination pattern. As a next
and substantial generalization we are going to incorporate semantics
for creating as well as deleting dynamics, in particular of type~A and
of type~B, consistently. This will enable, e.g., creation of a
stand-by $\McPal$ when the original $\McPal$ is busy with a first
migration: the stand-by can then initiate a different migration, even
before the first has finished.  As Paradigm's processes can model both
ICT activities and business activities, the McPal pattern is
particularly promising for addressing all kinds of alignment
situations between business and ICT and moreover for addressing
general evolution of ICT and business in tandem,
cf.~\cite{MBOWG07:ecsa}.

By means of ParADE, a modeling and animation environment for Paradigm
models, PhD work by Andries Stam, first migration examples have been
implemented and tested. A preliminary, but promising
result~\cite{foclasa08} has been obtained in translating Paradigm into
the process algebra~ACP.
%% ~\cite{BW90}. 
With its coupling to the mCRL2 toolkit~\cite{JFGDagstuhl},
state-of-the-art modelchecking of Paradigm models, in particular of
migration trajectories, comes into reach.


